Disjunctive bases: normal forms and model theory for modal logics

We present the concept of a disjunctive basis as a generic framework for normal forms in modal logic based on coalgebra. Disjunctive bases were defined in previous work on completeness for modal fixpoint logics, where they played a central role in the proof of a generic completeness theorem for coalgebraic mu-calculi. Believing the concept has a much wider significance, here we investigate it more thoroughly in its own right. We show that the presence of a disjunctive basis at the "one-step" level entails a number of good properties for a coalgebraic mu-calculus, in particular, a simulation theorem showing that every alternating automaton can be transformed into an equivalent nondeterministic one. Based on this, we prove a Lyndon theorem for the full fixpoint logic, its fixpoint-free fragment and its one-step fragment, and a Uniform Interpolation result, for both the full mu-calculus and its fixpoint-free fragment. We also raise the questions, when a disjunctive basis exists, and how disjunctive bases are related to Moss' coalgebraic "nabla" modalities. Nabla formulas provide disjunctive bases for many coalgebraic modal logics, but there are cases where disjunctive bases give useful normal forms even when nabla formulas fail to do so, our prime example being graded modal logic. We also show that disjunctive bases are preserved by forming sums, products and compositions of coalgebraic modal logics, providing tools for modular construction of modal logics admitting disjunctive bases. Finally, we consider the problem of giving a category-theoretic formulation of disjunctive bases, and provide a partial solution.

==> sec-jw-theorem.tex <==
\section{A  Janin-Walukiewicz theorem via disjunctive bases}

Our goal in this section is to prove a coalgebraic generalization of the
Janin-Walukiewicz theorem for the modal $\mu$-calculus, using disjunctive bases.
In joint work with Fatemeh Seifan~\cite{enqv:expr17}, we have previously proved
such results using
automata for coalgebraic MSO and assuming some conditions on a version of the
modal one-step language extended with monadic second-order quantifiers.
The result that we present here uses only a condition on the modal one-step
language itself, and avoids the use of automata for the MSO-language.
This also means that we get a new proof of the Janin-Walukiewicz theorem for
the $\mu$-calculus, which proceeds via a strong form of bisimulation quantifiers.

In this section we will not assume that the coalgebraic type functor $\funT$
preserves inclusion maps, since the notion of a \emph{support} will play an
important role and so we want to be as explicit about it as possible.
Instead we make the weaker assumption that $\funT$ preserves all monics in
$\Set$.\footnote{%
   This is a harmless assumption as we can modify $\funT$ into a functor
   $\funT'$ that does preserve monics, only by changing its value on the empty
   set.
   Since there is only one coalgebra on the empty set, the collection of
   coalgebras for $\funT$ and $\funT'$ is the same.
   }

\begin{definition}%
\label{d:supp}
Given $\xi \in \funT X$, a \emph{support} of $\xi$ is a subset $X' \subseteq X$
such that there is some $\xi' \in \funT X'$ with $\funT \iota (\xi') = \xi$,
where $\iota : X' \to X$ is the inclusion map.
Since $\funT$ preserves monics, if $X'$ is a support of $\xi \in \funT X$ then
there is a \emph{unique} $\xi' \in \funT X'$ with $\funT \iota (\xi') = \xi$;
we shall denote this object by  $\xi \vert_{X'}$.

We say that $\funT$ \emph{naturally admits minimal supports} if there is a natural
transformation $\mathsf{sup} : \fun \Rightarrow \funP$ such that % chktex 35
$\mathsf{sup}_X(\xi)$ is the smallest support for $\xi$ for any $\xi \in % chktex 35
\funT X$.
\end{definition}

It follows by results of Gumm~\cite{gumm05:from} that a finitary functor naturally
admits minimal supports iff it weakly preserves \emph{pre-images}; thus for
instance, all finitary functors preserving weak pullbacks have the property.
Functors lacking this property include the monotone neighborhoud functor
$\funM$. The reason that we require the map $\mathsf{sup}$ to be natural is to ensure that it gives rise to a predicate lifting for the functor $\funT$. In particular, if a modal signature contains this predicate lifting then we can reason about supports within the object language. More generally: % chktex 35

\begin{definition}
If $\funT$ naturally admits minimal supports, we say that the modal signature $\Lambda$
for $\funT$ has the \emph{support modality} if there is a positive one-step
formula $\supbox a$ such that a one-step model $(X,\xi,m)$ satisfies $\supbox
a$ iff $v \satzero a$ for all $v \in \mathsf{sup}_X(\xi)$. % chktex 35
\end{definition}

For example, the powerset functor has the support modality $\Box$ witnessed
by the identity natural transformation on $\funP$.
The multi-set functor has the support modality $\Box^1 $ witnessed by the
natural transformation mapping $\xi \mapsto \{v \in X \mid \xi(v) > 0\}$ for
$\xi \in \funB X$.
More generally, it follows by the earlier mentioned results of
Gumm~\cite{gumm05:from} that any Lyndon complete modal signature for a finitary
functor that weakly preserves pre-images has the support modality.

Coalgebraic monadic second-order logic was introduced in~\cite{enqv:expr17}.

\begin{definition}
Given a modal signature $\Lambda$,
we define the syntax of the monadic second-order logic $\mathtt{MSO}_\Lambda$ by
the following grammar:
\[
\varphi :=
  \sr(p) \mid p \subseteq q
  \mid \lambda(p,q_1,..,q_n) \mid
  \varphi \vee \varphi \mid \neg \varphi \mid \exists p. \varphi
\]
where $\lambda$ is any $n$-place monotone predicate lifting in $\Lambda$ and
$p,q,q_1,\dots,q_n \in Var$.
For the semantics, let $(\mathbb{S},s)$ be a pointed  $\fun$-model, where $\bbS
= (S,\si,V)$.
We define the satisfaction relation ${\sat} \subseteq S \times
\mathtt{MSO}_\Lambda$ as follows:
\[\begin{array}{lll}
   (\mathbb{S},s) \sat \sr(p)
   & \text{iff} & V(p) = \{s\}
\\ (\mathbb{S},s)\sat p \subseteq q
   & \text{iff} & V(p) \subseteq V(q),
\\ (\mathbb{S},s) \sat \lambda(p, q_1,\dots,q_n)
   & \text{iff} & \sigma (v)\in \lambda_S(V(q_1),..,V(q_n)) \text{ for all } v \in V(p)
\\ (\mathbb{S},s) \sat \exists p .\varphi
   & \text{iff} & (S,\sigma,V[p \mapsto Z],s)\sat  \varphi, \text{ some } Z \sse S,
\end{array}\]
while we use standard clauses for the Boolean connectives.
\end{definition}

The problem we address in this section is to compare the expressive power of
coalgebraic monadic second-order logic to that of the coalgebraic $\mu$-calculus.

\begin{definition}
A formula $\varphi \in \mathtt{MSO}_\Lambda$ is \emph{bisimulation invariant} if
for all pointed $\funT$-models $(\bbS,s)$ and $(\bbS',s')$ it holds that
$\bbS,s \sat \varphi$
and $(\bbS,s) \beheq (\bbS',s')$ implies $\bbS',s' \sat \varphi$.
\end{definition}

Our goal is to prove the following theorem:

\begin{thm}%
\label{t:jw}
Suppose that $\funT$ naturally admits minimal supports, and that the modal signature
$\Lambda$ admits a uniform disjunctive basis, and has the support modality.
Then $\muML_\Lambda$ is the bisimulation invariant fragment of
$\mathtt{MSO}_\Lambda$, i.e., a formula of $\mathtt{MSO}_\Lambda$ is bisimulation invariant if and only if it is equivalent to a formula in $\muML_\Lambda$.
\end{thm}

The assumption that $\funT$ naturally admits minimal supports and
$\Lambda$ has the support modality is used to ensure that the we can express hidden first-order quantifiers such as in formulas $p \subseteq q$, ``up to behavioural equivalence'', in the language $\muML_\Lambda$.
The following observation provides the easy part of the theorem  --- we omit the
proof, which is routine.

\begin{prop}%
\label{p:mu-to-mso}
Let $\La$ be a set of monotone predicate liftings for the set functor $\fun$.
There is an inductively defined translation ${(\cdot)}^{\diamond}$ mapping any
formula $\phi \in \muMLLa$ to a semantically equivalent formula
$\phi^{\diamond}\in \mathtt{MSO}_\Lambda$.
\end{prop}

For the opposite direction, we need to slightly refine the construction from the
proof of Proposition~\ref{p:dj1}.
Fix a uniform disjunctive basis $\D$.
For every one-step frame $(X,\xi)$, we first make use of the assumptions that $\funT$ naturally admits minimal supports, and then let
\[
    f_\xi : (X_*,\xi_*)  \to (\mathsf{sup}_X(\xi),\xi \vert_{\mathsf{sup}_X(\xi)}) % chktex 35
\]
be the one-step frame
morphism witnessing that $\D$ is a uniform disjunctive basis, for the case of
the one-step frame $(\mathsf{sup}_X(\xi),\xi \vert_{\mathsf{sup}_X(\xi)})$. % chktex 35
Then $\iota_{\mathsf{\mathsf{sup}_X(\xi)},X} \circ f_\xi : (X_*,\xi_*) \to % chktex 35
(X,\xi)$ is also a one-step frame morphism.
Note furthermore that the map $f_\xi : X_* \to \mathsf{sup}_X(\xi)$ has to be % chktex 35
surjective, since otherwise $f_\xi[X_*]$ is a support for
$\funT(\iota_{\mathsf{\mathsf{sup}_X(\xi)},X} \circ f_\xi)(\xi_*)$ in $X$ which % chktex 35
is smaller than $\mathsf{\mathsf{sup}_X(\xi)}$, which contradicts the definition. % chktex 35

\begin{definition}
Given a pointed $\funT$-model $(\bbS,s)$, let the \emph{supporting Kripke frame}
be $(S,R_{\bbS})$ where $v R_{\bbS} w$ iff $w \in
\mathsf{sup}_S(\sigma(v))$. % chktex 35
\end{definition}

The following proposition is similar to Proposition~\ref{p:dj1} in Section~\ref{s:sim}, but note that there are a few crucial differences. In particular, conditions (1) -- (3) state conditions for the supporting Kripke frames involved in the construction, which only make sense when $\funT$ naturally admits minimal supports. Furthermore, we are making use of the existence of a \emph{uniform} disjunctive basis to ensure that the construction is dependent only on the input $\funT$-model $(\bbS,s)$, and cannot depend on an automaton $\bbA$ as an extra parameter. % chktex 8


\begin{prop}
There is a construction that provides, for every $\funT$-model $(\bbS,s)$, a
pre-image $f_\bbS : (\bbS_*,s_*) \to (\bbS,s)$ such that:
\begin{enumerate}
    \item the structure $(S_{*},R_{\bbS_{*}})$ is a tree rooted at $s_{*}$;
    \item the map $f_\bbS$ is both a $\funT$-model homomorphism and a morphism of the supporting Kripke frames;
    \item $f_{\bbS}$ maps $S_{*}$ surjectively onto the set of points in $\bbS$ that are reachable from $s$ via the reflexive transitive closure of the support relation $R_{\bbS}$;
    \item any disjunctive $\Lambda$-automaton $\bbA$ accepts $(\bbS,s)$ iff it strongly accepts $(\bbS_*,s_*)$.
\end{enumerate}
\end{prop}
\begin{proof}
The construction of the pre-image  $f_\bbS : (\bbS_*,s_*) \to (\bbS,s)$
essentially follows the construction used in the proof of Proposition 5.7
in~\cite{enqv:expr17}, from which the first two conditions follow.
Given that we have constructed the covers
$\iota_{\mathsf{\mathsf{sup}_X(\xi)},X} \circ f_\xi : (X_*,\xi_*) \to (X,\xi)$ % chktex 35
so that they factor epi-monically through the natural inclusion of supports
$\iota_{\mathsf{\mathsf{sup}_X(\xi)},X} : \mathsf{sup}_X(\xi) \to X$, it is easy % chktex 35
to verify condition (3).
For condition (4), the argument closely follows that in the proof of
Proposition~\ref{p:dj1} in Section~\ref{s:sim}. We omit the details.
\end{proof}

\begin{proofof}{Theorem~\ref{t:jw}}
We provide a recursive translation $t : \mathtt{MSO}_\Lambda(\Prop) \to \muML_\Lambda(\Prop)$ such that for any formula $\varphi$ and any pointed $\funT$-model $(\bbS,s)$, we have:
\begin{equation}
\label{eq:dagger}
\bbS_*,s_* \sat \varphi \text{ iff } \bbS,s \sat t(\varphi).
\end{equation}
If $\varphi$ is bisimulation invariant, it then follows that
$\bbS,s \sat \varphi$ iff $\bbS_*,s_* \sat \varphi$ iff  $\bbS,s \sat t(\varphi)$, so that $\varphi$ is equivalent to $t(\varphi)$ as required.

The translation is defined as follows:

\begin{center}
\begin{tabular}{|l|l|} % chktex 44
\hline % chktex 44
    $\varphi$             & $t(\varphi)$
\\ \hline % chktex 44
   $\sr(p)$
   & $p \wedge \nu x. \supbox( x \land \neg p)$ \\
   $p \subseteq q$
   & $\nu x. (p \to q) \land \supbox x$
\\
   $\lambda(p,q_1,\dots,q_n)$
   & $\nu x. (p \to \hs_\lambda(q_1,\dots,q_n)) \land \supbox x$
\\
   $\alpha \vee \beta $
   & $t(\alpha ) \vee t(\beta)$
\\
   $\neg \alpha $
   & $\neg t(\alpha ) $
\\
   $\exists p. \alpha $
   & $\widetilde{\exists} p. t(\alpha) $
\\ \hline % chktex 44
\end{tabular}
\end{center}
where the map $\widetilde{\exists }p : \muML_\Lambda(\Prop p) \to \muML_\Lambda(\Prop)$ is defined precisely as in Section~\ref{s:ui}.
We can now prove the equivalence~\eqref{eq:dagger} by induction on the complexity
of formulas of $\mathtt{MSO}_\Lambda$.
The first three atomic cases for $\sr(p)$, $p \subseteq q$ and $\lambda(p,q_1,\dots,q_n)$ can be checked by routine verification, where the proofs for the first two cases uses the fact that the map $f_\bbS$ maps the points of $\bbS_*$ surjectively onto the points in $\bbS$, the second case additionally uses the fact that $\bbS_*$ is constructed so that its supporting Kripke frame is a tree rooted at $s_*$ (see~\cite{enqv:expr17} for details), and the case for $\lambda(p,q_1,\dots,q_n)$ uses the fact that $f_\bbS$ is a $\funT$-model homomorphism. The induction steps for boolean connectives are trivial. Finally, the proof for the crucial case of $\exists p. \varphi$ closely follows that of Proposition~\ref{p:ui1}, so we omit the details.
\end{proofof}


%\subsection{The supported companion functor}
%
%
%\begin{definition}
%Given a one-step $\underline{\fun}$-frame $(X,S,\xi)$ where $(S,\xi) \in \underline{\fun} X$, let $\xi\vert_S$ denote the unique object $\xi'$ in $\funT S$ such that $\funT \iota_{S,X} (\xi') = \xi$.
%\btbs
%\item We assume that $\funT$ preserves injective maps.
%\etbs
%\end{definition}
%
%\begin{prop}
%Suppose that the modal signature $\Lambda$ for $\funT$ admits a uniform disjunctive basis. Then so does the modal signature $\underline{\Lambda}$ for $\underline{\fun}$.
%\end{prop}
%
%\begin{proof}
%Let $\D$ be the uniform disjunctive basis for $\Lambda$. We define the collection of formulas $\underline{\D}(A)$ for a given set of variables $A$ to be the set of all disjunctions of formulas of the form:
%$$ \delta \wedge (\gdia b_1 \wedge \dots \wedge \gdia b_n \wedge \gbox(b_1 \vee \dots \vee b_n) )$$
%where $\delta \in \D(A)$. It suffices to check that these formulas are disjunctive, with uniformly chosen witnessing one-step frame morphisms, since a routine verification then shows that the appropriate distributive laws hold so that $\underline{\D}$ is indeed a disjunctive basis.
%
%Given a one-step $\underline{\fun}$-frame $(X,S,\xi)$ where $(S,\xi) \in \underline{\fun} X$, let $f : (S',\xi') \to (S,\xi \vert_S)$ be the one-step frame morphism for the frame $(S,\xi\vert_S)$ witnessing that $\D$ is a uniform disjunctive basis. We can assume without loss of generality that the map $f$ is surjective onto $S$, since otherwise it is easy to rectify this.
%\btbs
%\item Provide the details?
%\etbs
%Define $\gamma \in \funT (S' \times \omega)$ by setting such that $\funT \pi(\gamma) = \xi'$ where $\pi$ is the (surjective) projection map $\pi : X \times \omega \to X$. We consider the one-step $\underline{\funT}$-frame morphism:
%$$\iota_{S,X} \circ f \circ \pi : (S' \times \omega,S' \times \omega, \gamma) \to (X,S,\xi)$$
%This is indeed a one-step $\underline{\funT}$-frame morphism since the maps $\pi : S' times \omega \to S'$, $f : S' \to S$ are surjective and $\iota_{S,X}$ is just the identity on $S$.
%
%Now let $ \delta \wedge (\gdia b_1 \wedge \dots \wedge \gdia b_n \wedge \gbox(b_1 \vee \dots \vee b_n) )$, and let $m : X \to $





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:

